Neural Camera Models

Modern computer vision has moved beyond the domain of internet photo collections and into the physical world, guiding camera-equipped robots and autonomous cars through unstructured environments. To enable these embodied agents to interact with real-world objects, cameras are increasingly being used as depth sensors, reconstructing the environment for a variety of downstream reasoning tasks. Machine-learning-aided depth perception, or depth estimation, predicts for each pixel in an image the distance to the imaged scene point. While impressive strides have been made in depth estimation, significant challenges remain: (1) ground truth depth labels are difficult and expensive to collect at scale, (2) camera information is typically assumed to be known, but is often unreliable and (3) restrictive camera assumptions are common, even though a great variety of camera types and lenses are used in practice. In this thesis, we focus on relaxing these assumptions, and describe contributions toward the ultimate goal of turning cameras into truly generic depth sensors.

==> depth_field_networks/figures/architecture_features.tex <==
\begin{figure}[t!]
%\vspace{-3mm}
\renewcommand{\arraystretch}{0.95}
\centering
\subfloat[Depth architecture features.]{
\label{fig:stereo_results}
\raisebox{13mm}{
    \begin{tabular}{l|cccccc}
        \toprule
        Method &
        CV & 
        EP &
        BA &
        OF &
        SN &
        Realtime
 \\
        \toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & & & & & & \textcolor{red}{\xmark}\\
BA-Net (5-view) [2019]~\cite{tang2018ba} & & & \checkmark & & & \textcolor{red}{\xmark} \\
Neural-RGBD [2019]~\cite{liu2019neural} & \checkmark & & & \\ 
DeepV2D [2020]~\cite{deepv2d} & \checkmark & & \checkmark &  \\  
DELTAS [2020]~\cite{sinha2020depth} & & & &  \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  & & \checkmark & &  \\
DRN (refined) [2021]~\cite{ke2021deep} & & & \checkmark & \checkmark \\
MVDepth [2018]~\cite{???} & & & &  \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & &   \\
NAS [2020]~\cite{nas} & & & & \\
EST [2021]~\cite{long2021multi} & \checkmark &  & &  \\
DRN [2021]~\cite{ke2021deep} & &  & & \checkmark &  \\
        \bottomrule
GSR & & & & & & \textcolor{green}{\checkmark}
    \end{tabular}
}
\label{tab:depth_scannet_stereo}
}

\caption{Baseline methods are specialized to depth estimation and use traditional architectures elements.  The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
}
\label{fig:arch_features}
\end{figure}




==> depth_field_networks/figures/ddad_results.tex <==


\begin{figure}[t!]
\centering
\subfloat{
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_gt_rgb.png}
} \\ %\vspace{-4mm}
\subfloat{
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
} \\ %\vspace{-4mm}
\subfloat{
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
}
\caption{DDAD view and depthh synthesis results. Top: ground-truth images. Middle: predicted RGB values. Bottom: Predicted depth maps.}
\end{figure}

==> depth_field_networks/figures/encodings.tex <==


% \begin{figure}[t!]
% \centering
% \subfloat[Image Embeddings]{
% \label{fig:rgb_embeddings}
% \includegraphics[width=0.4\textwidth]{figures/files/image_embeddings.png}
% }
% \subfloat[Camera Embeddings]{
% \label{fig:cam_embeddings}
% \includegraphics[width=0.5\textwidth]{figures/files/camera_embeddings.png}
% }
% \caption{
% Embeddings used to encode and decode information. Image embeddings are used \emph{only} at the encoding stage, jointly with camera embeddings. During the decoding stage, only camera embeddings are used to produce synthesized depth and images from novel viewpoints.
% }
% \label{fig:encodings}
% \end{figure}

==> depth_field_networks/figures/extrapolation.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb0.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb1.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb2.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb3.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb4.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb5.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb6.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb7.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/rgb8.png}}
\vspace{-3mm} \\ 
\subfloat[$t$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel0.png}}
\hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel1.png}}
\hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel2.png}}
\hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel3.png}}
\hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel4.png}}
\hspace{0.1mm}
\subfloat[$t+5$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel5.png}}
\hspace{0.1mm}
\subfloat[$t+6$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel6.png}}
\hspace{0.1mm}
\subfloat[$t+7$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel7.png}}
\hspace{0.1mm}
\subfloat[$t+8$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/extrapolation/novel8.png}}
\caption{Depth extrapolation.}
\end{figure}

==> depth_field_networks/figures/forecast_all.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% \rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(0)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(1)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(2)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(3)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(4)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(5)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(6)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(7)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(8)_gt.png}} 
% \\ 
% \rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(0)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(1)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(2)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(3)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(4)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(5)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(6)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(7)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(8)_gt_viz.png}} 
% \\ 
% \rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(8)_pred_viz.png}} 
% \\ 
% \rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
% \subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(8)_pred_viz.png}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\vspace{2mm} \\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(0)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(1)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(2)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(3)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(4)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(5)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(6)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(7)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_rgb(8)_gt.png}} 
\\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(0)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(1)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(2)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(3)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(4)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(5)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(6)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(7)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(8)_gt_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth_valid_gt(8)_pred_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
\subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3033/0000003033_depth(8)_pred_viz.png}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% \vspace{2mm} \\ 
% \rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(0)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(1)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(2)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(3)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(4)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(5)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(6)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(7)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(8)_gt.png}} 
% \\ 
% \rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(0)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(1)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(2)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(3)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(4)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(5)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(6)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(7)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(8)_gt_viz.png}} 
% \\ 
% \rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(8)_pred_viz.png}} 
% \\ 
% \rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
% \subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(8)_pred_viz.png}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% \vspace{2mm} \\ 
% \rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(0)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(1)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(2)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(3)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(4)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(5)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(6)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(7)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_rgb(8)_gt.png}} 
% \\ 
% \rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(0)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(1)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(2)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(3)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(4)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(5)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(6)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(7)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(8)_gt_viz.png}} 
% \\ 
% \rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth_valid_gt(8)_pred_viz.png}} 
% \\ 
% \rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
% \subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/977/0000000977_depth(8)_pred_viz.png}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\vspace{2mm} \\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(0)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(1)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(2)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(3)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(4)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(5)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(6)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(7)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_rgb(8)_gt.png}} 
\\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(0)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(1)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(2)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(3)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(4)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(5)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(6)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(7)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(8)_gt_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth_valid_gt(8)_pred_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
\subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/3017/0000003017_depth(8)_pred_viz.png}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\vspace{2mm} \\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(0)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(1)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(2)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(3)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(4)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(5)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(6)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(7)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_rgb(8)_gt.png}} 
\\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(0)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(1)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(2)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(3)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(4)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(5)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(6)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(7)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(8)_gt_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth_valid_gt(8)_pred_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
\subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/1380/0000001380_depth(8)_pred_viz.png}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{ScanNet depth extrapolation examples}, using DeFiNe. In each example, image and camera information from frames at $[t-5,\dots,t-1]$ is encoded, and depth maps corresponding to camera locations at $[t,\dots,t+8]$ are decoded, using only camera information. For each timestep, we show sparse projected ground-truth depth maps (third row), and dense predicted depth maps (fourth row). Our DeFiNe architecture is able to extrapolate from encoded information to fill in missing parts of the scene.}
\label{fig:extra_additional}
\end{figure}

==> depth_field_networks/figures/forecast_all_backup.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
\rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/26/0000000026_rgb(0)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/26/0000000026_rgb(1)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/26/0000000026_rgb(2)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/26/0000000026_rgb(3)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/26/0000000026_rgb(4)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{depth_field_networks/figures/files/forecast/26/0000000026_rgb(5)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(6)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(7)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(8)_gt.png}} 
\\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(0)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(1)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(2)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(3)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(4)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(5)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(6)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(7)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(8)_gt_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(8)_pred_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
\subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(8)_pred_viz.png}}
% \caption{Depth extrapolation.}
% \end{figure}
% \vspace{-2mm} 
% \\
% % \begin{figure}[t!]
% % \captionsetup[subfloat]{labelformat=empty}
% \rotatebox{90}{\hspace{1.5mm} \tiny{RGB}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(0)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(1)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(2)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(3)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(4)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(5)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(6)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(7)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(8)_gt.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Depth GT}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(0)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(1)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(2)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(3)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(4)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(5)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(6)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(7)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(8)_gt_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Projection}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(8)_pred_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Predicted}} \!
% \subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(8)_pred_viz.png}}
% % \caption{Depth extrapolation.}
% % \end{figure}
% \vspace{-2mm} \\
% % \begin{figure}[t!]
% % \captionsetup[subfloat]{labelformat=empty}
% \rotatebox{90}{\hspace{1.5mm} \tiny{RGB}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(0)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(1)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(2)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(3)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(4)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(5)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(6)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(7)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(8)_gt.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Depth GT}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(0)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(1)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(2)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(3)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(4)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(5)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(6)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(7)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(8)_gt_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Projection}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(8)_pred_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Predicted}} \!
% \subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(8)_pred_viz.png}}
\caption{\textbf{ScanNet depth extrapolation examples}, using our proposed GSR architecture. In each example, information from frames at $[t-8,\dots,t-1]$ is encoded, and depth maps corresponding to camera locations at $[t,\dots,t+8]$ are decoded. RGB images and ground-truth depth maps are displayed only for comparison, and not used in these experiments. For each timestep, we show projected ground-truth depth maps (third row), and predicted depth maps (fourth row). Our GSR architecture is able to correctly extrapolate from encoded information to fill in missing parts of the scene.}
\end{figure}

==> depth_field_networks/figures/iib_comparison_error.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/0000001682_rgb(0)_gt.png}} \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/gt_1682.png}} \!
\subfloat{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/pred_1682.png}}  \!
\subfloat{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/diff_image_1682.png}} \! 
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/pred_1682.png}}  \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/diff_image_1682.png}}
\\
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/0000000168_rgb(0)_gt.png}} \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/gt_168.png}} \!
\subfloat{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/pred_168.png}}  \!
\subfloat{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/diff_image_168.png}} \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/pred_168.png}}  \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/diff_image_168.png}}
\\ 
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/0000004754_rgb(0)_gt.png}} \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/gt_4754.png}} \!
\subfloat{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/pred_4754.png}}  \!
\subfloat{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/diff_image_4754.png}}  \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/pred_4754.png}}  \!
\subfloat{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/diff_image_4754.png}}
\\ 
\subfloat[Input Image]{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/0000001940_rgb(0)_gt.png}} \!
\subfloat[GT depth]{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/define/gt_1940.png}} \!
\subfloat[DeFiNe depth]{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/pred_1940.png}} \!
\subfloat[DeFiNe error]{\includegraphics[width=0.17\textwidth,height=1.4cm]{figures/files/iib_comparison/define/diff_image_1940.png}} \!
\subfloat[IIB depth]{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/pred_1940.png}} \!
\subfloat[IIB error]{\includegraphics[width=0.16\textwidth,height=1.4cm]{figures/files/iib_comparison/iib/diff_image_1940.png}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Qualitative comparison of DeFiNe} relative to the IIB~\cite{yifan2021input} baseline.  
Our architecture improves depth estimation quality in (i) smooth and textureless areas, (ii) far away regions, and (iii) image boundaries and depth discontinuities.
%The first column is the stereo pair, the second column is the DeFiNe prediction for the left camera and its error map, the next column is the IIB prediction and its error map, and final column is the GT depth map.
%Note that the depth errors for the IIB model around image boundaries and depth discontinuities.  
%Our DeFiNe architecture is able to correctly predict depth in these regions.
}
\label{fig:iib}
%\vspace{-5mm}
\end{figure}

==> depth_field_networks/figures/interpolation.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\vspace{-5mm} \\ 
\subfloat[$t-4$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t-3$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t-2$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t-1$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}}
\caption{Depth interpolation.}
\label{fig:depth_synthesis}
\end{figure}

==> depth_field_networks/figures/scannet_stereo_lowres.tex <==



\begin{figure}[t!]
%\vspace{-3mm}
\renewcommand{\arraystretch}{0.95}
\centering
\subfloat[Depth estimation results.]{
\label{fig:stereo_results}
\raisebox{13mm}{
    \begin{tabular}{l|cccc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        \small{Sq.Rel}$\downarrow$ &
        RMSE$\downarrow$ &
        $\delta_{1.25}$$\uparrow$
 \\
        \toprule
        DPSNet~\cite{dpsnet} & 0.126 & --- & 0.314 & ---  \\
        NAS~\cite{nas} & 0.107 & --- & 0.281 & ---  \\
        IIB~\cite{yifan2021input} & 0.116 & --- & 0.281 & 0.908  \\
        \midrule
        \textbf{\MethodAcronym} & \textbf{0.089} & \textbf{0.037} & \textbf{0.232} & \textbf{0.915} \\
        \bottomrule
    \end{tabular}
}
\label{tab:depth_scannet_stereo}
}
\hspace{1mm}
\subfloat[Virtual depth estimation results.]{
\label{fig:virtual_results}
    \includegraphics[width=0.4\textwidth, height=2.6cm]{depth_field_networks/figures/files/virtual_error2.png}
    \label{fig:virtual_error}
}
\caption{\textbf{Depth estimation results on ScanNet-Stereo}. As shown in (a), we outperform other methods by a large margin. In (b) we report depth estimation results on virtual cameras, using different values of $\sigma_v$ at training and test time. 
}
\label{fig:depth_scannet_stereo}
\end{figure}





% \begin{figure}[t!]
% \small
% \centering
% \hspace{5mm}
% \subfloat[View synthesis results]{
%     \begin{tabular}{l|ccc}
%         \toprule
%         \textbf{Method} &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ &
%         LPIPS$\downarrow$ \\
%         \toprule
%         \midrule
%         \textbf{Ours (T)} & 0.714 & 23.810 & - \\
%         \textbf{Ours (C)} & 0.684 & 22.919 & - \\
%         \bottomrule
%     \end{tabular}
% }
% \\
% \subfloat[Depth degradation when rendering depth from different viewpoints.]{
%     \includegraphics[width=0.4\linewidth]{figures/files/virtual_error.png}
% }
% \hspace{5mm}

% % \subfloat[Depth synthesis results]{
% %     \begin{tabular}{l|ccc}
% %         \toprule
% %         \textbf{Method} &
% %         Abs.Rel$\downarrow$ &
% %         RMSE$\downarrow$ &
% %         $\delta_{1.25}$$\uparrow$ \\
% %         \toprule
% %         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- \\
% %         NAS~\cite{nas} & 0.1070 & 0.2807 & --- \\
% %         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 \\
% %         \midrule
% %         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 \\
% %         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 \\
% %         \bottomrule
% %     \end{tabular}
% % }

% \subfloat[Depth synthesis results]{
%     \begin{tabular}{l|ccccc}
%         \toprule
%         \textbf{Method} &
%         Abs.Rel$\downarrow$ &
%         RMSE$\downarrow$ &
%         $\delta_{1.25}$$\uparrow$ &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ \\
%         \toprule
%         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- & &  \\
%         NAS~\cite{nas} & 0.1070 & 0.2807 & --- & &  \\
%         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 & &  \\
%         \midrule
%         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 & & \\
%         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 & &  \\
%         \bottomrule
%     \end{tabular}
% }

% \caption{ScanNet-Stereo results, for depth and view synthesis.}
% \end{figure}

==> depth_field_networks/figures/scannet_stereo_psnr.tex <==



\begin{figure}[t!]
\renewcommand{\arraystretch}{0.95}
\centering
\subfloat[Depth estimation and view synthesis results.]{
\label{fig:stereo_results}
\raisebox{13mm}{
    \begin{tabular}{l|ccc|cc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        RMSE$\downarrow$ &
        $\delta_{1.25}$$\uparrow$ &
        SSIM$\uparrow$ &
        PSNR$\uparrow$ \\
        \toprule
        DPSNet~\cite{dpsnet} & 0.126 & 0.314 & --- & --- & ---  \\
        NAS~\cite{nas} & 0.107 & 0.281 & --- & --- & ---  \\
        IIB~\cite{yifan2021input} & 0.116 & 0.281 & 0.908 & --- & ---  \\
        \midrule
        \textbf{GSR} & \textbf{0.093} & \textbf{0.246} & \textbf{0.911} & \textbf{0.828} & \textbf{27.727} \\
        \bottomrule
    \end{tabular}
}
\label{tab:depth_scannet_stereo}
}
\hspace{1mm}
\subfloat[Virtual depth estimation results.]{
\label{fig:virtual_results}
    \includegraphics[width=0.36\textwidth, height=3cm]{depth_field_networks/figures/files/virtual_error.png}
    \label{fig:virtual_error}
}
\caption{\textbf{Depth estimation results on ScanNet-Stereo}. As shown in (a), we outperform other methods by a large margin. In (b) we report depth estimation results on virtual cameras, using different values of $\sigma_v$ at training and test time. 
}
\label{fig:depth_scannet_stereo}
\end{figure}





% \begin{figure}[t!]
% \small
% \centering
% \hspace{5mm}
% \subfloat[View synthesis results]{
%     \begin{tabular}{l|ccc}
%         \toprule
%         \textbf{Method} &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ &
%         LPIPS$\downarrow$ \\
%         \toprule
%         \midrule
%         \textbf{Ours (T)} & 0.714 & 23.810 & - \\
%         \textbf{Ours (C)} & 0.684 & 22.919 & - \\
%         \bottomrule
%     \end{tabular}
% }
% \\
% \subfloat[Depth degradation when rendering depth from different viewpoints.]{
%     \includegraphics[width=0.4\linewidth]{figures/files/virtual_error.png}
% }
% \hspace{5mm}

% % \subfloat[Depth synthesis results]{
% %     \begin{tabular}{l|ccc}
% %         \toprule
% %         \textbf{Method} &
% %         Abs.Rel$\downarrow$ &
% %         RMSE$\downarrow$ &
% %         $\delta_{1.25}$$\uparrow$ \\
% %         \toprule
% %         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- \\
% %         NAS~\cite{nas} & 0.1070 & 0.2807 & --- \\
% %         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 \\
% %         \midrule
% %         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 \\
% %         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 \\
% %         \bottomrule
% %     \end{tabular}
% % }

% \subfloat[Depth synthesis results]{
%     \begin{tabular}{l|ccccc}
%         \toprule
%         \textbf{Method} &
%         Abs.Rel$\downarrow$ &
%         RMSE$\downarrow$ &
%         $\delta_{1.25}$$\uparrow$ &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ \\
%         \toprule
%         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- & &  \\
%         NAS~\cite{nas} & 0.1070 & 0.2807 & --- & &  \\
%         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 & &  \\
%         \midrule
%         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 & & \\
%         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 & &  \\
%         \bottomrule
%     \end{tabular}
% }

% \caption{ScanNet-Stereo results, for depth and view synthesis.}
% \end{figure}

==> depth_field_networks/figures/scannet_synthesis.tex <==


% \begin{figure}[t!]
% \centering
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/scannet_pcl.png}
% }
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% } \\
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% } \\
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% }
% \caption{DDAD view and depthh synthesis results. Top: ground-truth images. Middle: predicted RGB values. Bottom: Predicted depth maps.}
% \end{figure}

% \begin{figure}[t!]
% \begin{tabular}{cc}
% % \vspace{-30mm}
% % \subfloat{
% % \raisebox{20mm}{\multirow{2}{*}{
% % \vspace{0mm}
% \vspace{10mm}
% \multirow{3}{*}{
% % \raisebox{20mm}{\multirow{2}{*}{
% \includegraphics[width=0.3\columnwidth,height=3cm]{figures/files/scannet_pcl.png}
% % }
% }
% % \\
% % % }
% % % \vspace{-3mm}
% % % \vspace{-30mm}
% % % \\
% % % % \vspace{-30mm}
% % \subfloat[qwer]{
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % }
% % }
% % }
% % }
% & 
% % \raisebox{20mm}{
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% &
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% &
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% % }
% \end{tabular}
% \caption{}
% \end{figure}


% \begin{figure}[t!]
% % \vspace{-30mm}
% % \raisebox{20mm}{\multirow{2}{*}{
% % \subfloat{
% % \raisebox{20mm}{\multirow{2}{*}{
% \subfloat{
% \includegraphics[width=0.3\columnwidth]{figures/files/scannet_pcl.png}
% }
% % }
% % \vspace{-3mm}
% % \vspace{-30mm}
% % \\
% % % \vspace{-30mm}
% % \subfloat[qwer]{
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % }
% % }
% % }
% % }
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% % &
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% }
% % \end{tabular}
% \caption{}
% \end{figure}



\begin{figure}[t!]
\begin{tabular}{cc}
% \vspace{10mm}
\raisebox{7mm}{\multirow{3}{*}{
\includegraphics[width=0.3\columnwidth,height=3cm]{figures/files/scannet_pcl.png}
}}
& 
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
\\
&
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
\\
&
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{depth_field_networks/figures/files/ddad_depth.png}
\end{tabular}
\caption{Depth and view synthesis results on the ScanNet-Stereo dataset.}
\end{figure}

==> depth_field_networks/figures/scannet_temporal.tex <==



% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|c|c|c|c|c|ccc|c}
        \toprule
        \textbf{Method} &
        CV & EP & BA & OF & SN &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
        \toprule
\multicolumn{6}{l}{\textbf{With test-time refinement}} \\
\toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & & & & & &
0.2310 & 0.5200 & 0.7610 & 110  \\
BA-Net (5-view) [2019]~\cite{tang2018ba} & & & \checkmark & & &  
%0.091 & 0.058 & 0.223 & \underline{95} \\
- & - & - & \underline{95} \\
Neural-RGBD [2019]~\cite{liu2019neural} & \checkmark & & & & &   
0.1013 & 0.0502 & 0.2500 & 195 \\
%DeepV2D [2020]~\cite{deepv2d} & \checkmark & & \checkmark & & &   
%- & - & - & 690 \\
%\textbf{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
DELTAS [2020]~\cite{sinha2020depth} & & & & & &   
0.0915 & 0.0327 & 0.2390 & \textbf{90} \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  & & \checkmark & & & &   
%0.073 & 0.037 & 0.217 & 2400 \\
- & - & - & 2400 \\
DRN (refined) [2021]~\cite{ke2021deep} & & & \checkmark & \checkmark & &   
- & - & - & 168 \\
%\underline{0.058} & \underline{0.018} & \textbf{0.162} & 168 \\
\midrule
\multicolumn{6}{l}{\textbf{Without test-time refinement}} \\
\midrule
MVDepth [2018]~\cite{???} & & & & & &   
0.1167 & 0.0596 & 0.3236 & - \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & & & &   
0.2080 & 0.3180 & 0.7420 & - \\
NAS [2020]~\cite{nas} & & & & & &   
0.0941 & 0.0417 & 0.2703 & - \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
EST [2021]~\cite{long2021multi} & \checkmark &  & & & &   
0.0812 & 0.0298 & 0.2199 & 71 \\
%\midrule
DRN [2021]~\cite{ke2021deep} & &  & & \checkmark & &   
%\underline{0.068} & \underline{0.026} & \textbf{0.178} & - \\
- & - & - & - \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
% | DEPTH|GT(0_0)_0                |  0.063   |  0.024   |  0.194   |  0.093   |  8.987   |  0.952   |  0.990   |  0.998   |  0.910   | 
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}} \\
\midrule
MVDepth [2018]~\cite{???} & \checkmark & & & & &   
0.2213 & 0.2401 & 0.5154 & - \\
DPSNet [2019]~\cite{dpsnet} & \checkmark & & & & &   
0.1963 & 0.1970 & 0.4625 & 225 \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
NAS [2020]~\cite{nas} & & \checkmark & & & \checkmark &   
0.1631 & 0.1023 & 0.3791 & - \\
EST [2021]~\cite{yifan2021input} & \checkmark &  & & & &   
0.1465 & 0.0729 & 0.3382 & 71 \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet}. We separate methods that include test-time refinement (e.g. windowed bundle adjustment) from those that, similar to ours, do not refine at test time. We also include zero-shot transfer results to 7~Scenes. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
%Results trained on the full Scannet dataset, trained and evaluated with window size of [-X,X].  The $\dagger$ indicates test-time optimization, while GRS is only a forward pass.
}
%\vspace{-3mm}
\label{fig:depth_scannet_temporal}
\end{table}


        %  & 0.196 & 0.197 & 0.463  \\
        %  & 0.163 & 0.102 & 0.379   \\
        %  & 0.147 & 0.073 & 0.338   \\
        % \midrule
        % \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\



==> depth_field_networks/figures/scannet_temporal_deepv2d_align.tex <==
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|ccc|c}
        \toprule
        \textbf{Method} &
        \small{Abs.\ Rel}$\downarrow$ &
        Sq.\ Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{ScanNet test split} \cite{tang2018ba}} \\
\midrule
DeMoN [2017]~\cite{ummenhofer2017demon} &
0.231 & 0.520 & 0.761 & 110  \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & 
0.208 & 0.318 & 0.742 & - \\
BA-Net [2019]~\cite{tang2018ba} &
0.091 & 0.058 & 0.223 & 95 \\
CVD [2020]~\cite{luo2020consistent} &   
0.073 & 0.037 & 0.217 & 2400 \\
DeepV2D [2020]~\cite{deepv2d} &  
\underline{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} & 
\textbf{0.047} & 0.024 & \textbf{0.164} & \textbf{30} \\
\midrule
\textbf{\MethodAcronym} ($128 \times 192$)&
0.059 & 0.022 & 0.184 &  \underline{49} \\
\textbf{\MethodAcronym} ($240 \times 320$) &
\underline{0.057} & \underline{0.019} & 0.178 &  78 \\

\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}~\cite{shotton2013scene}} \\
\midrule
DeMoN [2017]~\cite{ummenhofer2017demon} &  
0.389 & 0.420 & 0.855 & 110 \\
NeuralRGBD [2019]~\cite{liu2019neural} &
0.176 & 0.112 & 0.441 & 202 \\
DPSNet [2019]~\cite{dpsnet} &  
0.199 & 0.142 & 0.438  & 322 \\
DeepV2D [2020]~\cite{deepv2d} &  
0.437 & 0.553 & 0.869  & 347 \\
CNMNet [2020]~\cite{long2020occlusion} &   
0.161 & 0.083 & 0.361 & 80 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} &  
0.155 & 0.104 & 0.347 & \textbf{30} \\
EST [2021]~\cite{yifan2021input} &  
\underline{0.118} & \underline{0.052} & \underline{0.298} & 71 \\
\midrule
\textbf{\MethodAcronym} & 
\textbf{0.100} & \textbf{0.039} & \textbf{0.253} &  \underline{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet and 7~Scenes}. 
\MethodAcronym is competitive with other state-of-the-art methods on ScanNet, and outperforms all published methods in zero-shot transfer to 7~Scenes by a large margin.
}
%\vspace{-10mm}
\label{tab:depth_scannet_temporal}
\end{table}



==> depth_field_networks/figures/scannet_temporal_deev2d_checkmarks.tex <==

% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|cccc|ccc|c}
        \toprule
        \textbf{Method} &
        CV & EP & BA & SN &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{ScanNet test split} \cite{tang2018ba}} \\
\midrule
DeMoN$^\dagger$ [2017]~\cite{ummenhofer2017demon} & & & & & 
0.231 & 0.520 & 0.761 & 110  \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & & &  
0.208 & 0.318 & 0.742 & - \\
BA-Net$^\dagger$ (5-view) [2019]~\cite{tang2018ba} & & & \textcolor{red}{\checkmark} & & 
0.091 & 0.058 & 0.223 & 95 \\
CVD$^\dagger$ [2020]~\cite{luo2020consistent} & & \textcolor{red}{\checkmark} & & &   
0.073 & 0.037 & 0.217 & 2400 \\
DeepV2D$^\dagger$ [2020]~\cite{deepv2d} & \textcolor{red}{\checkmark}  & & \textcolor{red}{\checkmark} & &   
\underline{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} & & & & \textcolor{red}{\checkmark} &  
\textbf{0.047} & 0.024 & \textbf{0.164} & \textbf{30} \\
\midrule
\textbf{GSR} & & & & & 
0.059 & \underline{0.020} & 0.183 &  \underline{49} \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}~\cite{shotton2013scene}} \\
\midrule
DeMoN [2017]~\cite{ummenhofer2017demon} &  & & & & 
0.389 & 0.420 & 0.855 & 110 \\
% MVSNet [2018]~\cite{yao2018mvsnet} &   
% 0.234 & 0.190 & 0.508 & 1050 \\
NeuralRGBD [2019]~\cite{liu2019neural} & \textcolor{red}{\checkmark}  & & & & 
0.176 & 0.112 & 0.441 & 202 \\
% MVDNet [2018]~\cite{wang2018mvdepthnet} &  
% 0.193 & 0.235 & 0.459 & \underline{48} \\
DPSNet [2019]~\cite{dpsnet} & \textcolor{red}{\checkmark}  & & & & 
0.199 & 0.142 & 0.438  & 322 \\
DeepV2D [2020]~\cite{deepv2d} & \textcolor{red}{\checkmark}  & & \textcolor{red}{\checkmark} & &  
0.437 & 0.553 & 0.869  & 347 \\
CNMNet [2020]~\cite{long2020occlusion} & \textcolor{red}{\checkmark} & & & &    
0.161 & 0.083 & 0.361 & 80 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} & & & & \textcolor{red}{\checkmark} &   
0.155 & 0.104 & 0.347 & \textbf{30} \\
EST [2021]~\cite{yifan2021input} & \textcolor{red}{\checkmark} & & & &    
\underline{0.118} & \underline{0.052} & \underline{0.298} & 71 \\
\midrule
\textbf{GSR} & & & & & 
\textbf{0.100} & \textbf{0.039} & \textbf{0.253} &  \underline{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet and 7~Scenes}. 
The symbol $^\dagger$ indicates the use of test-time optimization. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), and SDF volumes (SV).
}
%\vspace{-10mm}
\label{fig:depth_scannet_temporal}
\end{table}



==> depth_field_networks/figures/scannet_temporal_scaled.tex <==



% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|ccc|c}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
        \toprule
\multicolumn{6}{l}{\textbf{With test-time refinement}} \\
\toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & 
0.231 & 0.520 & 0.761 & 110  \\
BA-Net (5-view) [2019]~\cite{tang2018ba} &  
0.091 & 0.058 & 0.223 & \underline{95} \\
Neural-RGBD [2019]~\cite{liu2019neural} &  
0.097 & 0.050 & 0.249 & 195 \\
DeepV2D [2020]~\cite{deepv2d} & 
\textbf{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
DELTAS [2020]~\cite{sinha2020depth} & 
0.092 & 0.033 & 0.234 & \textbf{90} \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  &  
0.073 & 0.037 & 0.217 & 2400 \\
DRN (refined) [2021]~\cite{ke2021deep} &  
\underline{0.058} & \underline{0.018} & \textbf{0.162} & 168 \\
\midrule
\multicolumn{6}{l}{\textbf{Without test-time refinement}} \\
\midrule
MiDas-v2 [2019]~\cite{ranftl2020towards} & 
0.208 & 0.318 & 0.742 & - \\
EST [2021]~\cite{long2021multi} &  
0.081 & 0.030 & 0.220 & 71 \\
%\midrule
DRN [2021]~\cite{ke2021deep} &  
\underline{0.068} & \underline{0.026} & \textbf{0.178} & - \\
\textbf{GSR} & & & & & &  
\textbf{0.063} & \textbf{0.024} & \underline{0.194} &  \textbf{49} \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}} \\
\midrule
DPSNet [2019]~\cite{dpsnet} & 
0.196 & 0.197 & 0.463 & 225 \\
NAS [2020]~\cite{nas} & 
0.163 & 0.102 & 0.379 & - \\
EST [2021]~\cite{yifan2021input} &  
\underline{0.147} & \underline{0.073} & \underline{0.338} & 71 \\
\textbf{GSR} & 
\textbf{0.106} & \textbf{0.044} & \textbf{0.267} &  \textbf{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet}. We separate methods that include test-time refinement (e.g. windowed bundle adjustment) from those that, similar to ours, do not refine at test time. We also include zero-shot transfer results to 7~Scenes. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
%Results trained on the full Scannet dataset, trained and evaluated with window size of [-X,X].  The $\dagger$ indicates test-time optimization, while GRS is only a forward pass.
}
\vspace{-3mm}
\label{fig:depth_scannet_temporal}
\end{table}


        %  & 0.196 & 0.197 & 0.463  \\
        %  & 0.163 & 0.102 & 0.379   \\
        %  & 0.147 & 0.073 & 0.338   \\
        % \midrule
        % \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\



==> depth_field_networks/figures/scannet_temporal_unscaled.tex <==



% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|c|c|c|c|c|ccc|c}
        \toprule
        \textbf{Method} &
        CV & EP & BA & OF & SN &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
        \toprule
\multicolumn{6}{l}{\textbf{With test-time refinement}} \\
\toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & & & & & &
0.2310 & 0.5200 & 0.7610 & 110  \\
BA-Net (5-view) [2019]~\cite{tang2018ba} & & & \checkmark & & &  
%0.091 & 0.058 & 0.223 & \underline{95} \\
- & - & - & \underline{95} \\
Neural-RGBD [2019]~\cite{liu2019neural} & \checkmark & & & & &   
0.1013 & 0.0502 & 0.2500 & 195 \\
%DeepV2D [2020]~\cite{deepv2d} & \checkmark & & \checkmark & & &   
%- & - & - & 690 \\
%\textbf{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
DELTAS [2020]~\cite{sinha2020depth} & & & & & &   
0.0915 & 0.0327 & 0.2390 & \textbf{90} \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  & & \checkmark & & & &   
%0.073 & 0.037 & 0.217 & 2400 \\
- & - & - & 2400 \\
DRN (refined) [2021]~\cite{ke2021deep} & & & \checkmark & \checkmark & &   
- & - & - & 168 \\
%\underline{0.058} & \underline{0.018} & \textbf{0.162} & 168 \\
\midrule
\multicolumn{6}{l}{\textbf{Without test-time refinement}} \\
\midrule
MVDepth [2018]~\cite{???} & & & & & &   
0.1167 & 0.0596 & 0.3236 & - \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & & & &   
0.2080 & 0.3180 & 0.7420 & - \\
NAS [2020]~\cite{nas} & & & & & &   
0.0941 & 0.0417 & 0.2703 & - \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
EST [2021]~\cite{long2021multi} & \checkmark &  & & & &   
0.0812 & 0.0298 & 0.2199 & 71 \\
%\midrule
DRN [2021]~\cite{ke2021deep} & &  & & \checkmark & &   
%\underline{0.068} & \underline{0.026} & \textbf{0.178} & - \\
- & - & - & - \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
% | DEPTH|GT(0_0)_0                |  0.063   |  0.024   |  0.194   |  0.093   |  8.987   |  0.952   |  0.990   |  0.998   |  0.910   | 
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}} \\
\midrule
MVDepth [2018]~\cite{???} & \checkmark & & & & &   
0.2213 & 0.2401 & 0.5154 & - \\
DPSNet [2019]~\cite{dpsnet} & \checkmark & & & & &   
0.1963 & 0.1970 & 0.4625 & 225 \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
NAS [2020]~\cite{nas} & & \checkmark & & & \checkmark &   
0.1631 & 0.1023 & 0.3791 & - \\
EST [2021]~\cite{yifan2021input} & \checkmark &  & & & &   
0.1465 & 0.0729 & 0.3382 & 71 \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet}. We separate methods that include test-time refinement (e.g. windowed bundle adjustment) from those that, similar to ours, do not refine at test time. We also include zero-shot transfer results to 7~Scenes. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
%Results trained on the full Scannet dataset, trained and evaluated with window size of [-X,X].  The $\dagger$ indicates test-time optimization, while GRS is only a forward pass.
}
%\vspace{-3mm}
\label{fig:depth_scannet_temporal}
\end{table}


        %  & 0.196 & 0.197 & 0.463  \\
        %  & 0.163 & 0.102 & 0.379   \\
        %  & 0.147 & 0.073 & 0.338   \\
        % \midrule
        % \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\



==> depth_field_networks/figures/seven_scenes.tex <==
\begin{figure}[t!]
%\begin{minipage}[c]{.5\textwidth}
\centering
\label{fig:sevenscenes_results}
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        Sq. Rel$\downarrow$ &
        RMSE$\downarrow$ \\
        \toprule
        DPSNet~\cite{dpsnet} & 0.196 & 0.197 & 0.463  \\
        NAS~\cite{nas} & 0.163 & 0.102 & 0.379   \\
        EST~\cite{yifan2021input} & 0.147 & 0.073 & 0.338   \\
        \midrule
        \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\
        \bottomrule
    \end{tabular}
%\end{minipage}%
%\begin{minipage}[c]{.5\textwidth}
\caption{\textbf{Depth estimation results on 7~Scenes}.  Models trained on the Scannet train set and tested on the 7~Scenes test set sequences.}
%}
\label{fig:depth_scannet_stereo}
%\end{minipage}
\end{figure}



==> depth_field_networks/figures/virtual.tex <==

\begin{figure}[t!]
\begin{tabular}{cc}
% \vspace{10mm}
\raisebox{9mm}{\multirow{2}{*}{
\includegraphics[width=0.3\columnwidth,height=2.5cm]{depth_field_networks/figures/files/scannet_pcl.png}
}}
& 
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/rgb.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/rgb1.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/rgb2.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/rgb3.png}
\\
&
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/depth.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/depth1.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/depth2.png}
    \includegraphics[width=0.15\textwidth]{depth_field_networks/figures/files/virtual/depth3.png}
\end{tabular}
\caption{Examples of virtual camera augmentations.}
\end{figure}

==> depth_field_networks/sections/supp_mat.tex <==
\section{Implementation Details}

\subsection{Training parameters}

We implemented our models using PyTorch,
% \footnote{Training and inference code will be made available upon publication.}, 
with distributed training across eight A100 GPUs. We used grid search to choose training parameters, that include: view synthesis weight $\lambda_s = 5.0$, virtual camera loss weight $\lambda_v=0.5$, virtual camera projection noise $\sigma_v = 0.25$, canonical jittering noise $\sigma_t=\sigma_r=0.1$, and batch size $b=32$ ($4$ per GPU). We use the AdamW optimizer~\cite{loshchilov2019decoupled}, with standard parameters $\beta_1=0.9$, $\beta_2=0.999$, a weight decay of $w=10^{-4}$, and an initial learning rate of $lr=2 \cdot 10^{-4}$. For our stereo experiments, we train for $200$ epochs, halving the learning rate every $80$ epochs. For our video experiments, we train for $100$ epochs, halving the learning rate every $40$ epochs. Higher-resolution fine-tuning is performed for $50$ epochs for stereo experiments, and $10$ epochs for video experiments, with $lr=2 \cdot 10^{-5}$.

\subsection{Architecture Details}

Following recent work~\cite{yifan2021input}, we use $K_o=20$ and $K_r=10$ as the number of Fourier frequencies for camera embeddings, with maximum resolution $\mu_o = \mu_r = 60$. Our encoder embeddings have dimensionality $C_e=960 + 186 = 1146$, due to the use of both image and camera information. Our decoder embeddings have dimensionality $C_d=186$, since only camera information is required to produce estimates. Our latent representation $\mathcal{R}$ is of dimensionality $2048 \times 512$. Input images are resized to $128 \times 192$, and following standard protocol~\cite{deepv2d} output depth maps are compared to ground-truth resized to $480 \times 640$. We use the following hyperparameters for our Perceiver~IO implementation: $1$ block, $1$ input cross-attention, $8$ self-attention layers (with $8$ heads) and $1$ output cross-attention.  Cross attention layers have only $1$ head. We found that larger Perceiver~IO models (i.e., with more blocks, number of heads, and self-/cross-attention layers) did not improve results and significantly increased training time. The latest developments in the Perceiver architecture~\cite{hier-perceiver} could be used to further improve performance and inference speed, and will be considered in future work.

\section{Canonical Jittering Test-time Ablation}

In Section 4.3 of the main text, we ablate the effects of using our proposed data augmentation techniques, designed to improve multi-view consistency in the learned latent representation. In Figure 4b we provide an additional experiment in which we vary the amount of virtual camera noise $\sigma_v$ at train and test time, and show that training at higher noise levels not only improves depth estimation performance at the target location (up to a certain value, of $\sigma_v=0.25$m), but also when decoding estimates from novel viewpoints. 

Here we perform a similar experiment targeting another proposed data augmentation technique: canonical jittering. Two different models were trained, with and without canonical jittering, and both were evaluated under different noise levels at test time.  Note that, while this augmentation does not change scene geometry, it changes the camera embeddings used for encoding and decoding information.
Results are presented in Table \ref{table:pose_jittering}. As we can see, the model trained with canonical jittering not only performs better when evaluating at the target location, but is also more robust to increasing levels of noise at test time. 
\input{tables/pose_jittering}


% Do we replicate information about the encoder here?

\section{Higher Resolution Fine-Tuning}
One of the main challenges of training Transformer-based architectures has been the $O(N^2)$ self-attention memory scaling with input size. 
This means that the resolution of recent models has been fairly limited (e.g. the view synthesis model of Sajjadi et al.~\cite{sajjadi2021scene} primarily trains on low-resolution images, with a highest resolution of $128 \times 176$), hindering their application to real-world scenes.  
Perceiver~IO decouples input resolution from the the learned latent representation, which enables training and real-time inference at higher resolutions~\cite{yifan2021input}.
In our experiments, we found it advantageous to train using a resolution curriculum, first at a lower resolution ($128 \times 192$), and then fine-tune at a higher resolution $(240 \times 320)$. Note that, because the camera parameters are also scaled to the proper resolution, the scene geometry does not change, only (a) the number of embeddings generated per camera, and (b) the image embeddings, since resolution changes image features.  Thus, training at lower resolutions enables the faster learning of our desired multi-view latent scene representation, which can then be fine-tuned at higher resolutions for further improvements.
%
As an alternative, we also experimented with the strategy of \textit{sampling} rays at higher resolution (similar to NeRF~\cite{mildenhall2020nerf} and SRT~\cite{sajjadi2021scene}). However, we found that this approach led to unstable training and longer convergence times. As future work, we plan to investigate how training and and inference can be scaled up to even higher resolutions. 
%, approximating.
%As future work we are experimenting with training at higher resolutions beyond $(240 \times 320)$.


%Interestingly, our model trained on $128 \times 192$ already achieves state-of-the-art results on Scannet-Stereo, outperforming IIB~\cite{yifan2021input} which is trained on $240 \times 320$ images.  We found that fine-tuning on larger images $(240 \times 320)$, which involve a larger number of ray queries, achieves superior results to training at the higher resolution from scratch.
% One of the main challenges of training Transformer-based architectures has been the $O(N^2)$ self-attention memory scaling with input size. This means that the resolution of recent models has been fairly limited (scene representation transformers~\cite{sajjadi2021scene} are trained on $176 \times 128$ images).  Perceiver~IO decouples input resolution from the the learned latent representation, which enables training in higher resolutions~\cite{yifan2021input}. has been trained at  higher resolutions -- IIB trains on stereo data at $240 \times 320$.  

%Given that self-attention in the Perceiver~IO architecture is decoupled from input resolution, we found it advantageous to fine-tune models at increasingly higher resolutions. Thus, we first train at $128 \times 192$ resolution, and then fine-tune the resulting model at $240 \times 320$ resolution for further improvement.

%We find it advantageous to train in a resolution curriculum, first at a lower resolution ($128 \times 192$) and then to fine-tune at a higher resolution $(240 \times 320)$.  The number of ray queries at lower resolutions is smaller and so the network has an easier time converging

\input{figures/iib_comparison_error}


%\section{Additional Qualitative Results}
\section{Comparison to IIB}
IIB~\cite{yifan2021input} is a recently proposed stereo depth estimation method that also uses a Perceiver~IO-based architecture.  Their major contribution is a geometrically-motivated epipolar inductive bias to encourage multi-view consistency. In Table 1 and Figure 4 of the main text, we show that our DeFiNe architecture significantly improves over the IIB baseline on the ScanNet-Stereo benchmark ($0.116$ vs. $0.089$ Abs. Rel.).  
%
Given that code and pre-trained models to replicate the IIB results are not available, we trained a model following the instructions in~\cite{yifan2021input}, achieving similar performance as reported in the paper. 

Some qualitative examples from this model are depicted in Figure \ref{fig:iib}, as well as examples from our DeFiNe architecture. As we can see, our proposed 3D augmentations and joint view synthesis learning also lead to significant qualitative improvements over IIB results. In particular, we consistently perform better in smooth and textureless areas, as well as far away regions and depth discontinuities. We attribute this behavior to an increase in scene diversity due to our contributions, that enables the learning of a more consistent multi-view latent scene representation.

%DeFiNe and color decoding lead to significant improvements over IIB both quantitatively and qualitatively, using no epipolar constraints.  Note that depth errors both around depth discontinuities and around image boundaries are smaller for DeFiNe than for IIB, we hypothesize that this is the effect of 3D augmentations which provide a richer, more multi-view consistent scene representation.

% \section{Scene Representation Ablations}
% DeFiNe learns a scene representation from a sequence from images.  We provide a further ablation comparing the stereo results of DeFiNe to a monocular variant, mapping only the source image to the source depth map with the same architecture. This section text TBD results of monocular training with 3D augmentations.
% % maybe further evidence for 3D augmentation
% \include{tables/monocular_ablations}

\section{Depth from Novel Viewpoints}

In Table \ref{tab:intra_extra} we provide numerical values to complement our depth interpolation and extrapolation experiments (Figures 7a and 7b from the main text). These experiments show that querying from our learned latent representation improves over the explicit projection of information from encoded views, while also enabling the estimation of dense depth maps from novel viewpoints. Similarly, in Figure \ref{fig:extra_additional} we provide additional qualitative examples of depth extrapolation to future timesteps, showing how DeFiNe can reconstruct unseen portions of the environment in a geometrically-consistent way.  

\input{depth_field_networks/tables/inter_extra}
\input{depth_field_networks/figures/forecast_all}
% \input{tables/extrapolation}




==> depth_field_networks/tables/ablation_psnr.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccc|cc}
\toprule
\multirow{2}{*}{\textbf{Variation}} &
\multicolumn{4}{c}{Depth} &
\multicolumn{2}{c}{View} \\
& 
Abs.Rel &
Sqr.Rel &
RMSE &
$\delta_{1.25}$ &
SSIM & 
PSNR \\
\toprule
Depth-Only & 0.098 & 0.046 & 0.257 & 0.902 & -- & -- \\
RGB-Only & -- & -- & -- & -- & 0.576 & 21.071 \\
\midrule
w/ Conv. RGB encoder & 0.114 & 0.058 & 0.294 & 0.866 & 0.644 & 23.151 \\
w/ 64-dim R18 RGB encoder & 0.104 & 0.049 & 0.270 & 0.883 & 0.675 & 23.859 \\
\midrule
w/o camera information & 0.229 & 0.157 & 0.473 & 0.661 & 0.606 & 16.924 \\
w/o global rays encoding & 0.097 & 0.047 & 0.261 & 0.897 & 0.788 & 26.267 \\
w/ equal loss weights & 0.095 & 0.047 & 0.259 & 0.908 & 0.736 & 24.621 \\
w/ epipolar cues~\cite{yifan2021input} & 0.094 & 0.048 & 0.254 & 0.905 & 0.798 & 26.998 \\
\midrule
w/o Augmentations & 0.117 & 0.060 & 0.291 & 0.870 & 0.741 & 24.758 \\
w/o Virtual Cameras & 0.104 & 0.058 & 0.268 & 0.891 & 0.770 & 25.274 \\
w/o Canonical Jittering & 0.099 & 0.046 & 0.261 & 0.897 & 0.788 & 26.267 \\
w/o Canonical Randomization & 0.096 & 0.044 & 0.253 & 0.905 & 0.792 & 26.284 \\
\midrule
% Ours ($T_1$) & 0.097 & 0.258 & 0.905 & 0.816 & 27.120  \\
\textbf{GSR} & \textbf{0.093} & \textbf{0.042} & \textbf{0.246} & \textbf{0.911} & \textbf{0.828} & \textbf{27.727} \\
\bottomrule
\end{tabular}
}
\caption{Ablation table for ScanNet-Stereo, using different GSR variations. } 
\label{tab:ablation}
%\vspace{-5mm}
\end{table*}



==> depth_field_networks/tables/depth_multi_camera.tex <==


\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|ccccc|ccc}
\toprule
& \multirow{2}{*}{\textbf{Camera}} &
\multicolumn{5}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& &
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Method}}}} 
& 01 & & & & & & & & \\
& 05 & & & & & & & & \\
& 06 & & & & & & & & \\
& 07 & & & & & & & & \\
& 08 & & & & & & & & \\
& 09 & & & & & & & & \\
\bottomrule
\end{tabular}
}
\caption{Placeholder multi-camera depth table.} 
\label{tab:depth_multi_camera}
\end{table*}




==> depth_field_networks/tables/depth_single_camera.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{5}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& 
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule
& & & & & & & & 
\\

\bottomrule

\end{tabular}
}
\caption{Placeholder single camera depth table.} 
\label{tab:depth_single_camera}
\end{table*}



==> depth_field_networks/tables/extrapolation.tex <==
\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccccccc}
% \toprule
% Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
% \midrule
% \% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
% \toprule
% Monodepth2 & 0.164 & 0.178 & 0.188 & 0.194 & 0.201 & 0.208 & 0.215 & 0.221 & 0.228 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GRS (projection) & 0.132 & 0.147 & 0.154 & 0.162 & 0.168 & 0.177 & 0.184 & 0.191 & 0.198 \\
% GRS (novel) & 0.131 & 0.144 & 0.151 & 0.158 & 0.165 & 0.172 & 0.178 & 0.184 & 0.190 \\
% \midrule
% \midrule
% GRS (novel, all) & 0.138 & 0.159 & 0.175 & 0.192 & 0.209 & 0.224 & 0.238 & 0.251 & 0.263 \\
% \bottomrule
\toprule
Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
\midrule
\% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
\toprule
Monodepth2 & 0.351 & 0.386 & 0.398 & 0.405 & 0.412 & 0.420 & 0.431 & 0.441 & 0.453 \\
PackNet & 0.327 & 0.358 & 0.378 & 0.391 & 0.400 & 0.406 & 0.420 & 0.428 & 0.436 \\
BTS & 0.315 & 0.331 & 0.357 & 0.377 & 0.392 & 0.401 & 0.413 & 0.424 & 0.429 \\
\midrule
DeFiNe (projection) & 0.258 & 0.276 & 0.288 & 0.298 & 0.311 & 0.323 & 0.331 & 0.340 & 0.348 \\
DeFiNe (query) & 0.237 & 0.260 & 0.271 & 0.280 & 0.289 & 0.298 & 0.307 & 0.317 & 0.326 \\
\midrule
\midrule
DeFiNe (query, all) & 0.326 & 0.370 & 0.405 & 0.438 & 0.468 & 0.495 & 0.520 & 0.543 & 0.563 \\
\bottomrule
\end{tabular}
}
\caption{Depth extrapolation (Abs.\ Rel).} 
\label{tab:extrapolation}
\end{table*}

==> depth_field_networks/tables/inter_extra.tex <==
\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\subfloat[Depth interpolation results.  
Frames at {[}$t-5,t+5${]} are encoded, and depth maps corresponding to camera locations at  {[}$t-4,\dots,t+4${]} are decoded.
%$
%$[t-5,t+5]$ 
]{
\begin{tabular}{l|ccccccccc}
\toprule
Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
\midrule
\% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
\toprule
Monodepth2~\cite{monodepth2} & 0.325 & 0.336 & 0.346 & 0.354 & 0.361 & 0.359 & 0.354 & 0.347 & 0.338 \\
PackNet~\cite{packnet}    & 0.305 & 0.318 & 0.330 & 0.341 & 0.344 & 0.344 & 0.336 & 0.327 & 0.338 \\
BTS~\cite{lee2019big}        & 0.296 & 0.306 & 0.320 & 0.329 & 0.334 & 0.326 & 0.327 & 0.319 & 0.303 \\
\midrule
DeFiNe (projection) & 0.226 & 0.239 & 0.251 & 0.259 & 0.268 & 0.261 & 0.254 & 0.244 & 0.231 \\
DeFiNe (query)      & 0.222 & 0.230 & 0.237 & 0.240 & 0.242 & 0.246 & 0.245 & 0.240 & 0.231 \\
\midrule
\midrule
DeFiNe (query, all) & 0.361 & 0.381 & 0.398 & 0.408 & 0.412 & 0.413 & 0.406 & 0.390 & 0.369 \\
\bottomrule
\end{tabular}
} \\
\subfloat[Depth extrapolation results. 
Frames at {[}$t-5,\dots,t-1${]} are encoded, and depth maps corresponding to camera locations at {[}$t,\dots,t+8${]} are decoded.
]{
\begin{tabular}{l|ccccccccc}
\toprule
Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
\midrule
\% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
\toprule
Monodepth2~\cite{monodepth2} & 0.351 & 0.386 & 0.398 & 0.405 & 0.412 & 0.420 & 0.431 & 0.441 & 0.453 \\
PackNet~\cite{packnet} & 0.327 & 0.358 & 0.378 & 0.391 & 0.400 & 0.406 & 0.420 & 0.428 & 0.436 \\
BTS~\cite{lee2019big} & 0.315 & 0.331 & 0.357 & 0.377 & 0.392 & 0.401 & 0.413 & 0.424 & 0.429 \\
\midrule
DeFiNe (projection) & 0.258 & 0.276 & 0.288 & 0.298 & 0.311 & 0.323 & 0.331 & 0.340 & 0.348 \\
DeFiNe (query) & 0.237 & 0.260 & 0.271 & 0.280 & 0.289 & 0.298 & 0.307 & 0.317 & 0.326 \\
\midrule
\midrule
DeFiNe (query, all) & 0.326 & 0.370 & 0.405 & 0.438 & 0.468 & 0.495 & 0.520 & 0.543 & 0.563 \\
\bottomrule
\end{tabular}
}
}
\caption{\textbf{Depth interpolation and extrapolation results}, on ScanNet (complementary to Figures 7a and 7b of the main text). On valid projected pixels, DeFiNe (query) outperforms the explicit projection of all considered single-frame baselines, and it also outperforms the explicit projection of its own estimates, obtained from encoded views (projection). Furthermore, it also enables the estimation of dense depth maps from novel viewpoints, which can be compared to the corresponding ground-truth from that location (query, all).} 
\label{tab:intra_extra}
%\vspace{-5mm}
\end{table*}

% \begin{table*}[t!]
% %\vspace{-4mm}
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}

% }
% \caption{Depth extrapolation (Abs.\ Rel).} 
% \label{tab:extrapolation}
% \end{table*}



==> depth_field_networks/tables/interpolation.tex <==
\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccccccc}
% \toprule
% Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
% \midrule
% \% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
% \toprule
% Monodepth2 & 0.168 & 0.179 & 0.186 & 0.193 & 0.200 & 0.196 & 0.190 & 0.183 & 0.172 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GRS (projection) & 0.138 & 0.146 & 0.155 & 0.162 & 0.165 & 0.163 & 0.158 & 0.150 & 0.139 \\
% GRS (novel) & 0.138 & 0.148 & 0.154 & 0.158 & 0.161 & 0.157 & 0.154 & 0.148 & 0.137 \\
% \midrule
% \midrule
% GRS (novel, all) & 0.150 & 0.159 & 0.166 & 0.172 & 0.176 & 0.174 & 0.171 & 0.163 & 0.153 \\
% \bottomrule
\toprule
Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
\midrule
\% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
\toprule
Monodepth2 & 0.325 & 0.336 & 0.346 & 0.354 & 0.361 & 0.359 & 0.354 & 0.347 & 0.338 \\
PackNet    & 0.305 & 0.318 & 0.330 & 0.341 & 0.344 & 0.344 & 0.336 & 0.327 & 0.338 \\
BTS        & 0.296 & 0.306 & 0.320 & 0.329 & 0.334 & 0.326 & 0.327 & 0.319 & 0.303 \\
\midrule
DeFiNe (projection) & 0.226 & 0.239 & 0.251 & 0.259 & 0.268 & 0.261 & 0.254 & 0.244 & 0.231 \\
DeFiNe (query)      & 0.222 & 0.230 & 0.237 & 0.240 & 0.242 & 0.246 & 0.245 & 0.240 & 0.231 \\
\midrule
\midrule
DeFiNe (query, all) & 0.361 & 0.381 & 0.398 & 0.408 & 0.412 & 0.413 & 0.406 & 0.390 & 0.369 \\
\bottomrule
\end{tabular}
}
\caption{Depth Interpolation.} 
\label{tab:interpolation}
\end{table*}

==> depth_field_networks/tables/monocular_ablations.tex <==
\begin{figure}[t!]
\centering
\label{fig:monocular_results}
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        % \small{Sq.Rel}$\downarrow$ &
        RMSE$\downarrow$ &
        $\delta_{1.25}$$\uparrow$ \\
        \toprule
        No Aug. & 0.149 & 0.078 & 0.806  \\
        3D Aug. & X & X & X  \\
        \midrule
        IIB~\cite{yifan2021input} & 0.116  & 0.281 & 0.908  \\
        \textbf{DeFiNe} & \textbf{0.089} & \textbf{0.232} & \textbf{0.915} \\
        \bottomrule
    \end{tabular}
\caption{Comparing \textbf{monocular depth} training to IIB and DeFiNe.}
\end{figure}

==> depth_field_networks/tables/pose_jittering.tex <==
\captionsetup[table]{skip=6pt}
\begin{table}[t!]
\renewcommand{\arraystretch}{1.1}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{|l|cccc|}
\toprule
\diagbox{Train}{Test} & 
$0.0$m  & 
$0.1$m &
$0.2$m &
$0.5$m
\\
\midrule
$0.0$m
&
$0.101$ & $0.202$ & $0.226$ & $0.291$ \\
$0.1$m
&
$0.097$ & $0.160$ & $0.184$ & $0.242$ \\ 
\bottomrule
\end{tabular}
}
\caption{\textbf{Effects of canonical jittering at train and test time}. The model trained with canonical jittering ($\sigma_t = \sigma_r = 0.1$m) not only performs better when evaluated at the target location ($\sigma_t = \sigma_r = 0.0$m), but is also more robust to different levels of canonical jittering at test time. The results shown are average Abs. Rel. of the two predicted stereo depths maps, without ground-truth scaling.}
%\vspace{-6mm}
\label{table:pose_jittering}
\end{table}

==> depth_field_networks/tables/scannet_viewsynth.tex <==
\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{5}{|c|}{Higher is better $\uparrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& 
PSNR &
LPIPS &
SSIM &
%RMSE$_{log}$ &
%SILog & 
%$\delta<1.25$ &
%$\delta<1.25^2$ &
%$\delta<1.25^3$\vspace{0.5mm}\\
\\
\toprule
PerspectiveNet & 13.986 & 0.426 & & & & & & 
\\

\bottomrule

\end{tabular}
}
\caption{View synthesis results on ScanNet.} 
\label{tab:scannet_view_synthesis}
\end{table*}



==> full_surround_monodepth/figures/both_qualitative.tex <==


\begin{figure*}[t!]
\centering
\subfloat{
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_01-rgb_7_04131fb1.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_05-rgb_7_89a852c0.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_06-rgb_7_0935301b.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_07-rgb_7_851143ac.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_08-rgb_7_2fff9472.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_09-rgb_7_570fd51a.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_01-inv_depth_7_fda4f2df.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_05-inv_depth_7_2bca48a2.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_06-inv_depth_7_40721199.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_07-inv_depth_7_ee4b9656.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_08-inv_depth_7_262042e2.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_09-inv_depth_7_9a32b507.png}
}
\vspace{-4mm}
\\
\subfloat[\emph{DDAD}]{
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_01-calc_normals_7_c7875beb.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_05-calc_normals_7_11c2267c.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_06-calc_normals_7_4d9ba474.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_07-calc_normals_7_338b1655.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_08-calc_normals_7_2ff0a179.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/ddad_qualitative/ddad-val-lidar-camera_09-calc_normals_7_8df871f3.png}
}
//
\subfloat{
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-rgb_1_40020b22.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-rgb_1_58b133e3.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-rgb_1_be6332ab.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-rgb_1_b91f6249.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-rgb_1_ee63df59.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-rgb_1_404be6c3.png}
}
\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-inv_depth_1_fc5d9c74.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-inv_depth_1_e7a451aa.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-inv_depth_1_14718541.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-inv_depth_1_556ac75b.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-inv_depth_1_36184bc7.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-inv_depth_1_66474543.png}
}
\vspace{-4mm}
\\
\subfloat[\emph{nuScenes}]{
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front-1480-calc_normals_1_74bf4dcd.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back-1480-calc_normals_1_9194d541.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_left-1480-calc_normals_1_2e9b09c7.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_back_right-1480-calc_normals_1_7e5eaccc.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_left-1480-calc_normals_1_b3d8e70b.png}
\includegraphics[width=0.16\linewidth]{full_surround_monodepth/images/nuscenes_qualitative/nuscenes_v1-val-lidar_top-cam_front_right-1480-calc_normals_1_a356d291.png}
}
\caption{\textbf{Self-Supervised depth estimation results} on the \emph{DDAD} and \emph{nuScenes} datasets using our proposed method, including surface normals calculated from the predicted depth maps.}
\label{fig:ddad_qualitative}
\end{figure*}


==> full_surround_monodepth/figures/ddad_non_overlapping.tex <==

\begin{figure}[t!]
\centering
\subfloat{
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/1/rgb.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/0/rgb.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/2/rgb.png}
}
%\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/1/rgb_context_1.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/0/rgb_context_1.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/2/rgb_context_1.png}
}
%\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/1/mask_1_0_0.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/0/mask_1_0_0.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/2/mask_1_0_0.png}
}
%\vspace{-4mm}
\\
\subfloat{
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/ddad_mask1.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/ddad_mask0.png}
\includegraphics[width=0.30\linewidth]{full_surround_monodepth/images/ddad_warps/ddad_mask2.png}
}
\caption{\textbf{Non-overlapping masks} calculated on the \textit{DDAD} dataset. \textbf{First and second rows:} Target and context frames. \textbf{Third row:} Temporal mask from context to target. \textbf{Fourth row:} Spatial mask from surrounding target images.}
\label{fig:non_overlapping_masks}
\end{figure}


==> full_surround_monodepth/figures/ddad_spatio_temporal.tex <==

\begin{figure}[t!]
\centering
\subfloat{
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/rgb1.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/rgb0.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/rgb2.png}
}
%\vspace{-3.5mm}
\\
\subfloat{
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_1.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_0.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_2.png}
}
%\vspace{-3.5mm}
\\
\subfloat{
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_context_1.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_context_0.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_context_2.png}
}
\caption{
\textbf{Examples of spatio-temporal photometric losses} on the \textit{DDAD} dataset. \textbf{Top row:} input RGB images. \textbf{Middle row:} Photometric losses considering only spatial contexts (Equation~\ref{eq:warp_spatial}). \textbf{Bottom row:} Photometric losses considering our proposed spatio-temporal contexts (Equation~\ref{eq:warp_multi}) from adjacent frames (forward and backwards).
}
\label{fig:pd_multicam}
\end{figure}


==> full_surround_monodepth/figures/pd_spatio_temporal.tex <==

\begin{figure}[t!]
\centering
\subfloat{
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/rgb1.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/rgb0.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/rgb2.png}
}
%\vspace{-3.5mm}
\\
\subfloat{
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_1.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_0.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_2.png}
}
%\vspace{-3.5mm}
\\
\subfloat{
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_context_1.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_context_0.png}
\includegraphics[width=0.32\linewidth]{full_surround_monodepth/images/ddad_photo/photo_cross_context_2.png}
}
\caption{
\textbf{Examples of spatio-temporal photometric losses} on the \textit{DDAD} dataset. \textbf{Top row:} input RGB images. \textbf{Middle row:} Photometric losses considering only spatial contexts (Equation~\ref{eq:warp_spatial}). \textbf{Bottom row:} Photometric losses considering our proposed spatio-temporal contexts (Equation~\ref{eq:warp_multi}) from adjacent frames (forward and backwards).
}
\label{fig:pd_multicam}
\end{figure}


==> full_surround_monodepth/figures/pd_warps.tex <==

\begin{figure*}[t!]
%\vspace{-5mm}
\begin{tabular}{cc}
\centering
\multirow{6}{*}{
%\hspace{-3mm}
\subfloat[Camera locations on the vehicle.]{
\raisebox{-51mm}{\includegraphics[width=0.28\linewidth,trim=0 350 0 0, clip]{images/pd_6cams.png}}}}
%\hspace{-5mm}
& 
\\
& 
\hspace{0.2mm}
\subfloat{
\textcolor{cyan}{\rule{1.93cm}{1mm}}
\textcolor{magenta}{\rule{1.92cm}{1mm}}
\textcolor{yellow}{\rule{1.92cm}{1mm}}
\textcolor{green}{\rule{1.92cm}{1mm}}
\textcolor{blue}{\rule{1.92cm}{1mm}}
\textcolor{red}{\rule{1.92cm}{1mm}}
}
%\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth,height=1.0cm]{images/ddad_photo/rgb0.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/rgb1.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/rgb2.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/rgb3.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/rgb4.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/rgb5.png}
}
%\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/warp_self_0.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/warp_self_1.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/warp_self_2.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/warp_self_3.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/warp_self_4.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/warp_self_5.png}
}
%\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/photo_self_0.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/photo_self_1.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/photo_self_2.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/photo_self_3.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/photo_self_4.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo/photo_self_5.png}
}
%\vspace{-4.5mm}
\\
& 
\hspace{0.1mm}
\subfloat{
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/warp_cross_0.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/warp_cross_1.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/warp_cross_2.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/warp_cross_3.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/warp_cross_4.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/warp_cross_5.png}
}
%\vspace{-4.5mm}
\\ 
&
\setcounter{subfigure}{1}
\subfloat[\textbf{First row:} Input RGB images. \textbf{Second and third rows:} Synthesized views from temporal contexts (Equation~\ref{eq:warp_mono}) and the corresponding photometric losses. \textbf{Third and fourth rows:} Synthesized views from surrounding cameras (Equation~\ref{eq:warp_spatial}) and the corresponding photometric losses (both overlaid).]{
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/photo_cross_0.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/photo_cross_1.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/photo_cross_2.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/photo_cross_3.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/photo_cross_4.png}
\includegraphics[width=0.11\linewidth]{full_surround_monodepth/images/ddad_photo2/photo_cross_5.png}
}
\end{tabular}
\caption{\textbf{Examples of spatial and temporal image warping} on the \textit{DDAD}  dataset. (a) shows the location of all six cameras, and (b) depicts the RGB images for each camera, alongside the synthesized images using information from other viewpoints and their corresponding photometric losses.}
\label{fig:pd_warps}
%\vspace{-5mm}
\end{figure*}


==> full_surround_monodepth/tables/both_scaling_small.tex <==

\begin{table}%
% \vspace{-1mm}
\centering
\small
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{0.3em}
\subfloat[DDAD]{
\begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{} &
    \multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{3-8}
    & 
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    \\
    \midrule
    Mono $-$ M
    & F
    & 0.184
    & 0.366
    & 0.448
    & 0.417
    & 0.426
    & 0.438
    \\
    Mono
    & F 
    & 0.139
    & 0.209
    & 0.236
    & 0.231
    & 0.247
    & 0.204
    \\
    \textbf{FSM}
    & F
    & \underline{0.131}
    & \underline{0.203}
    & \underline{0.226}
    & \textbf{0.223}
    & \textbf{0.240}
    & \underline{0.188}
    \\
    \midrule
    Mono
    & S
    & 0.143
    & 0.238
    & 0.265
    & 0.277
    & 0.276
    & 0.247
    \\
    \textbf{FSM}
    & S
    & 0.133
    & 0.212
    & 0.229
    & 0.231
    & \underline{0.246}
    & 0.194
    \\ 
    \midrule
    \textbf{FSM $-$ STC}
    & -
    & 0.133
    & 0.219
    & 0.246
    & 0.252
    & 0.259
    & 0.197
    \\
    \textbf{FSM $-$ PCC}
    & -
    & \underline{0.131}
    & 0.206
    & 0.228
    & 0.238 
    & 0.248
    & \underline{0.188}
    \\
    \textbf{FSM}
    & -
    & \textbf{0.130}
    & \textbf{0.201}
    & \textbf{0.224}
    & \underline{0.229}
    & \textbf{0.240}
    & \textbf{0.186}
    \\
    \bottomrule
\end{tabular}
}
\\
%\vspace{-2mm}
\subfloat[nuScenes]{
\begin{tabular}{l|c|cccccc}
    \toprule
    \multirow{2}{*}{} &
    \multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
    \multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
    \cmidrule{3-8}
    & 
    & \textit{Front}
    & \textit{F.Left}
    & \textit{F.Right}
    & \textit{B.Left}
    & \textit{B.Right}
    & \textit{Back}
    \\
    \midrule
    Mono
    & F 
    & 0.214
    & 0.304
    & 0.388
    & 0.314 
    & 0.438 
    & 0.304 
    \\
    \textbf{FSM}
    & F
    & 0.198
    & 0.297
    & \textbf{0.350}
    & \textbf{0.289} 
    & \textbf{0.392}
    & \underline{0.240}
    \\
    \midrule
    Mono
    & S
    & 0.251
    & 0.403 
    & 0.546
    & 0.429 
    & 0.616 
    & 0.321 
    \\
    \textbf{FSM}
    & S
    & 0.200 
    & 0.337 
    & 0.448
    & 0.354 
    & 0.521 
    & 0.267 
    \\ 
    \midrule
    \textbf{FSM $-$ STC}
    & -
    & 0.208
    & 0.382
    & 0.510
    & 0.393
    & 0.595
    & 0.258
    \\ 
    \textbf{FSM $-$ PCC}
    & -
    & \underline{0.187} 
    & \underline{0.291}
    & 0.392
    & 0.311
    & 0.448
    & 0.235
    \\ 
    \textbf{FSM}
    & -
    & \textbf{0.186}
    & \textbf{0.287}
    & \underline{0.375}
    & \underline{0.296}
    & \underline{0.418}
    & \textbf{0.221}
    \\
    \bottomrule
\end{tabular}
}
%\vspace{-2mm}
\caption{\textbf{Depth estimation results on multi-camera datasets}, using \emph{FSM} relative to the single-camera photometric loss (\emph{Mono}). In the scaling column, \emph{F} denotes per-frame median-scaling, and \emph{S} our proposed shared median-scaling. \emph{M} denotes the removal of masking (Sec.~\ref{sec:mask}), \emph{STC} the removal of spatio-temporal contexts (Sec.~\ref{sec:stc}), and \emph{PCC} the removal of pose consistency constraints (Sec.~\ref{sec:pcc}).}
\label{tab:both_scaling_small}
%\vspace{-3mm}
\end{table}

==> full_surround_monodepth/tables/ddad_ablation.tex <==

\captionsetup[table]{skip=6pt}

\begin{table}[t!]
%\vspace{-3mm}
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccc}
\toprule
\textbf{Method} & \textbf{Sup.} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}$ $\uparrow$
\\
\toprule
SuperDepth~\cite{superdepth} 
& $S$ & 0.112 & 0.875 & 4.958 & 0.852 \\
Monodepth2~\cite{godard2019digging} 
& $M$ & 0.115 & 0.903 & 4.863 & 0.877 \\
Monodepth2~\cite{godard2019digging} 
& $S$ & 0.109 & 0.873 & 4.960 & 0.864 \\
\midrule
Monodepth2~\cite{godard2019digging} 
& $M+S$ & \textbf{0.106} & \textbf{0.818} & 4.750 & \textbf{0.874} \\
Ours & $STC$ & 0.112 & 0.767 & \textbf{4.705} & 0.864 \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Ablation experiments on DDAD}, to validate the various components and design choices of our proposed architecture.}
\label{table:ddad_ablation}
%\vspace{-3mm}
\end{table}

==> full_surround_monodepth/tables/ddad_scaling.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc|cccccc}
\toprule
\multirow{2}{*}{\rotatebox{45}{\textbf{Method}}} &
\multirow{2}{*}{\rotatebox{45}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} &
\multicolumn{6}{|c}{$\delta < 1.25\uparrow$} \\
\cmidrule{3-14}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
\\
\midrule
Mono
& Indiv. 
& 0.139
& 0.209
& 0.236
& 0.231
& 0.247
& 0.204
& 0.832
& 0.709
& 0.673
& 0.686
& 0.660
& 0.695
\\
\textbf{MultiCam}
& Indiv.
& 0.131
& 0.203
& 0.226
& 0.223
& 0.240
& 0.188
& 0.840
& 0.716
& 0.687
& 0.693
& 0.670
& 0.714
\\
\midrule
Mono
& Shared
& 0.143
& 0.227
& 0.253
& 0.264
& 0.263
& 0.236
& 0.828
& 0.623
& 0.582
& 0.509
& 0.530
& 0.558
\\
\textbf{MultiCam}
& Shared
& 0.133
& 0.212
& 0.239
& 0.241
& 0.256
& 0.194
& 0.837
& 0.673
& 0.639
& 0.600
& 0.585
& 0.683
\\ 
\midrule
\textbf{MultiCam - STC}
& ---
& 0.133
& 0.219
& 0.246
& 0.252
& 0.259
& 0.197
& 0.830
& 0.627
& 0.599
& 0.552
& 0.554
& 0.674
\\
\textbf{MultiCam}
& ---
& 0.131
& 0.206
& 0.228
& 0.238 
& 0.248
& 0.188
& 0.831
& 0.669
& 0.650
& 0.594
& 0.587
& 0.687
\\
\bottomrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Mono (Standard)}}}} 
% & 01 & 0.139 & 3.023 & 13.835 & 0.234 & 22.782 & 0.832 & 0.937 & 0.970
% \\
% & 05 & 0.209 & 3.410 & 12.609 & 0.319 & 30.722 & 0.709 & 0.881 & 0.938
% \\
% & 06 & 0.236 & 3.827 & 12.097 & 0.344 & 33.294 & 0.673 & 0.860 & 0.928
% \\
% & 07 & 0.231 & 3.976 & 12.311 & 0.331 & 31.874 & 0.686 & 0.863 & 0.931
% \\
% & 08 & 0.247 & 3.776 & 11.449 & 0.354 & 33.996 & 0.660 & 0.850 & 0.925
% \\
% & 09 & 0.204 & 3.345 & 14.371 & 0.309 & 30.150 & 0.695 & 0.889 & 0.949
% \\

% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Mono (Shared)}}}} 
% & 01 & 0.143 & 3.133 & 13.875 & 0.237 & 23.029 & 0.828 & 0.935 & 0.970
% \\
% & 05 & 0.227 & 3.624 & 13.545 & 0.365 & 30.685 & 0.623 & 0.840 & 0.917
% \\
% & 06 & 0.253 & 4.197 & 13.324 & 0.400 & 33.375 & 0.582 & 0.821 & 0.905
% \\
% & 07 & 0.264 & 4.103 & 14.038 & 0.419 & 31.827 & 0.509 & 0.778 & 0.890
% \\
% & 08 & 0.263 & 3.856 & 12.739 & 0.419 & 34.001 & 0.530 & 0.795 & 0.896
% \\
% & 09 & 0.236 & 4.235 & 16.729 & 0.386 & 30.137 & 0.558 & 0.814 & 0.911
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Standard)}}}} 
% & 01 & 0.135 & 2.841 & 13.850 & 0.230 & 23.378 & 0.832 & 0.939 & 0.972
% \\
% & 05 & 0.207 & 3.239 & 12.608 & 0.320 & 30.793 & 0.705 & 0.879 & 0.938
% \\
% & 06 & 0.231 & 3.648 & 11.928 & 0.341 & 33.092 & 0.676 & 0.862 & 0.931
% \\
% & 07 & 0.225 & 3.804 & 12.341 & 0.330 & 31.804 & 0.688 & 0.863 & 0.930
% \\
% & 08 & 0.240 & 3.525 & 11.277 & 0.350 & 33.776 & 0.667 & 0.854 & 0.928
% \\
% & 09 & 0.200 & 3.379 & 14.934 & 0.312 & 30.450 & 0.694 & 0.887 & 0.948
% \\

% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Shared)}}}} 
% & 01 & 0.138 & 2.924 & 14.041 & 0.232 & 22.557 & 0.826 & 0.937 & 0.971
% \\
% & 05 & 0.218 & 3.363 & 13.172 & 0.351 & 30.966 & 0.655 & 0.848 & 0.923
% \\
% & 06 & 0.241 & 3.896 & 12.827 & 0.377 & 32.893 & 0.621 & 0.835 & 0.914
% \\
% & 07 & 0.249 & 3.761 & 13.289 & 0.384 & 32.133 & 0.580 & 0.818 & 0.908
% \\
% & 08 & 0.257 & 3.549 & 12.096 & 0.393 & 33.719 & 0.568 & 0.821 & 0.910
% \\
% & 09 & 0.205 & 3.629 & 15.419 & 0.334 & 30.211 & 0.668 & 0.865 & 0.936
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Multi (Aware)}}}} 
% & 01 & 0.137 & 3.027 & 14.220 & 0.237 & 22.596 & 0.821 & 0.934 & 0.970
% \\
% & 05 & 0.211 & 3.335 & 13.219 & 0.350 & 30.966 & 0.661 & 0.849 & 0.923
% \\
% & 06 & 0.231 & 3.844 & 12.860 & 0.375 & 32.893 & 0.639 & 0.835 & 0.912
% \\
% & 07 & 0.244 & 3.731 & 13.303 & 0.384 & 32.133 & 0.589 & 0.814 & 0.907
% \\
% & 08 & 0.247 & 3.512 & 12.140 & 0.390 & 33.719 & 0.584 & 0.824 & 0.910
% \\
% & 09 & 0.191 & 3.479 & 15.370 & 0.328 & 30.211 & 0.693 & 0.869 & 0.937
% \\

\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on DDAD}, using our proposed spatio-temporal photometric loss (\textit{Multi}) relative to the standard photometric loss (\textit{Mono}). The \textit{Standard} evaluation uses per-frame ground truth median scaling at test time; the \textit{Shared} evaluation uses our proposed per-sample ground-truth median scaling, using all six cameras; and the \textit{Aware} evaluation does not use median scaling at test time. Using the standard median scaling evaluation, our results are on-par with, our } 
\label{tab:depth_ddad}
\end{table*}





==> full_surround_monodepth/tables/ddad_scaling_small.tex <==

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc}
\toprule
\multirow{2}{*}{} &
\multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
\cmidrule{3-8}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{F.Right}
& \textit{B.Left}
& \textit{B.Right}
& \textit{Back}
\\
\midrule
Mono $-$ M
& F
& 0.184
& 0.366
& 0.448
& 0.417
& 0.426
& 0.438
\\
Mono
& F 
& 0.139
& 0.209
& 0.236
& 0.231
& 0.247
& 0.204
\\
\textbf{FSM}
& F
& \underline{0.131}
& \underline{0.203}
& \underline{0.226}
& \textbf{0.223}
& \textbf{0.240}
& \underline{0.188}
\\
\midrule
Mono
& S
& 0.143
& 0.238
& 0.265
& 0.277
& 0.276
& 0.247
\\
\textbf{FSM}
& S
& 0.133
& 0.212
& 0.229
& 0.231
& 0.246
& 0.194
\\ 
\midrule
\textbf{FSM $-$ STC}
& -
& 0.133
& 0.219
& \underline{0.246}
& 0.252
& 0.259
& 0.197
\\
\textbf{FSM $-$ PCC}
& -
& \underline{0.131}
& 0.206
& 0.228
& 0.238 
& 0.248
& \underline{0.188}
\\
\textbf{FSM}
& -
& \textbf{0.130}
& \textbf{0.201}
& \textbf{0.224}
& \underline{0.229}
& \textbf{0.240}
& \textbf{0.186}
\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Depth estimation results on DDAD}, using our proposed \emph{FSM} approach relative to the standard single-camera photometric loss (\emph{Mono}). In the scaling column, \emph{I} denotes per-frame median scaling, and \emph{S} our proposed shared median scaling.}
\label{tab:depth_ddad_small}
\end{table}





==> full_surround_monodepth/tables/nuscenes_scaling.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc|cccccc}
\toprule
\multirow{2}{*}{\rotatebox{45}{\textbf{Method}}} &
\multirow{2}{*}{\rotatebox{45}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} &
\multicolumn{6}{|c}{$\delta < 1.25\uparrow$} \\
\cmidrule{3-14}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
\\
\midrule
Mono
& Indiv. 
& 0.248
& 0.315
& 0.304 
& 0.304 
& 0.417 
& 0.398
& 0.727
& 0.629
& 0.659
& 0.712 
& 0.594
& 0.603
\\
\textbf{MultiCam}
& Indiv.
& 0.198
& 0.297
& 0.289 
& 0.240
& 0.392
& 0.350
& 0.748
& 0.643
& 0.670
& 0.731
& 0.620
& 0.631
\\
\midrule
Mono
& Shared
& 0.251
& 0.403 
& 0.429 
& 0.321 
& 0.616 
& 0.546
& 0.729
& 0.520
& 0.511
& 0.659 
& 0.497
& 0.508
\\
\textbf{MultiCam}
& Shared
& 0.200 
& 0.337 
& 0.354 
& 0.267 
& 0.521 
& 0.448
& 0.754
& 0.574
& 0.567
& 0.687 
& 0.549
& 0.558
\\ 
\midrule
\textbf{MultiCam - STC}
& ---
& 0.208
& 0.382
& 0.393
& 0.258
& 0.595
& 0.510
& 0.691
& 0.526
& 0.516
& 0.680
& 0.536
& 0.542
\\ 
\textbf{MultiCam}
& ---
& 0.187 
& 0.291
& 0.311
& 0.235
& 0.448
& 0.392
& 0.736
& 0.602
& 0.576
& 0.710
& 0.592
& 0.606
\\
\bottomrule


\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on nuScenes}, using our proposed spatio-temporal photometric loss (\textit{Multi} relative to the standard photometric loss (\textit{Mono}). The \textit{Standard} evaluation uses per-frame ground truth median scaling at test time; the \textit{Shared} evaluation uses our proposed per-sample ground-truth median scaling, using all six cameras; and the \textit{Aware} evaluation does not use median scaling at test time. Using the standard median scaling evaluation, our results are on-par with, our } 
\label{tab:depth_nuscenes}
\end{table*}





==> full_surround_monodepth/tables/nuscenes_scaling_small.tex <==

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccccc}
\toprule
\multirow{2}{*}{} &
\multirow{2}{*}{\rotatebox{90}{\textbf{Scaling}}} &
\multicolumn{6}{c}{Abs.Rel.$\downarrow$} \\
\cmidrule{3-8}
& 
& \textit{Front}
& \textit{F.Left}
& \textit{B.Left}
& \textit{Back}
& \textit{B.Right}
& \textit{F.Right}
\\
\midrule
Mono
& F 
& 0.214
& 0.304
& 0.294 
& 0.304 
& 0.408 
& 0.368
\\
\textbf{FSM}
& F
& 0.198
& 0.297
& 0.289 
& 0.240
& 0.392
& 0.350
\\
\midrule
Mono
& S
& 0.251
& 0.403 
& 0.429 
& 0.321 
& 0.616 
& 0.546
\\
\textbf{FSM}
& S
& 0.200 
& 0.337 
& 0.354 
& 0.267 
& 0.521 
& 0.448
\\ 
\midrule
\textbf{FSM $-$ STC}
& -
& 0.208
& 0.382
& 0.393
& 0.258
& 0.595
& 0.510
\\ 
\textbf{FSM $-$ PCC}
& -
& 0.187 
& 0.291
& 0.311
& 0.235
& 0.448
& 0.392
\\ 
\textbf{FSM}
& -
& \textbf{0.186}
& \textbf{0.287}
& 0.296
& 0.221
& 0.418
& 0.375
\\
\bottomrule

\end{tabular}
}
\caption{\textbf{Depth estimation results on nuScenes}, using FSM relative to the standard single-camera photometric loss. In the scaling column, \emph{I} denotes per-frame median scaling, and \emph{S} our proposed shared median scaling. \emph{M} refers to the removal of self-occlusion masks, and \emph{STC} to the removal of spatio-temporal constraints.}
\label{tab:depth_nuscenes_small}
\end{table}





==> full_surround_monodepth/tables/suppmat_networks.tex <==
\begin{table}[t!]%
\small
  \centering
\resizebox{0.84\linewidth}{!}{
\subfloat[][Depth Network \cite{monodepth2}.]{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}[b]{l|l|c|c|c}
\toprule
& \textbf{Layer Description} & \textbf{K} & \textbf{S} & \textbf{Out. Dim.} \\ 
\toprule
\multicolumn{5}{c}{\textbf{ResidualBlock (K, S)}} \\ 
\midrule
\#A & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU & K & 1 &  \\
\#B & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU & K & S &  \\
\toprule
\multicolumn{5}{c}{\textbf{UpsampleBlock (\#skip)}} \\ 
\midrule
\#C & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU $\shortrightarrow$ Upsample         & 3 & 1 & \\
\#D & Conv2d ($\#C \oplus \#skip$) $\shortrightarrow$ BN $\shortrightarrow$ ReLU  & 3 & 1 & \\
\toprule
\toprule
\#0 & Input RGB image & - & - & 3$\times$H$\times$W \\ 
\midrule
\multicolumn{5}{c}{\textbf{Encoder}} \\ \hline
\#1  & Conv2d $\shortrightarrow$ BN $\shortrightarrow$ ReLU   & 7 & 1 &  64$\times$H$\times$W \\
\#2  & Max. Pooling                 & 3 & 2 &  64$\times$H/2$\times$W/2 \\
\#3  & ResidualBlock (x2)           & 3 & 2 &  64$\times$H/4$\times$W/4 \\
\#4  & ResidualBlock (x2)           & 3 & 2 & 128$\times$H/8$\times$W/8 \\
\#5  & ResidualBlock (x2)           & 3 & 2 & 256$\times$H/16$\times$W/16 \\
\#6  & ResidualBlock (x2)           & 3 & 2 & 512$\times$H/32$\times$W/32 \\
\midrule
\multicolumn{5}{c}{\textbf{Depth Decoder}} \\ 
\midrule
\#7 & UpsampleBlock (\#5)    & 3 & 1 & 256$\times$H/16$\times$W/16 \\
\#8 & UpsampleBlock (\#4)    & 3 & 1 & 128$\times$H/8$\times$W/8 \\
\#9 & UpsampleBlock (\#3)    & 3 & 1 & 64$\times$H/4$\times$W/4 \\
\#10 & UpsampleBlock (\#2)   & 3 & 1 & 32$\times$H/2$\times$W/2 \\
\#11 & UpsampleBlock (\#1)   & 3 & 1 & 32$\times$H$\times$W \\
\#12 & Conv2d $\shortrightarrow$ Sigmoid  & 3 & 1 & 1$\times$H$\times$W \\
\bottomrule
\end{tabular}
\label{tab:netdepth}
}}
\\
\resizebox{0.84\linewidth}{!}{
\subfloat[][Pose Network \cite{zhou2018unsupervised}.]{
\begin{tabular}[b]{l|c|c|c|c}
\toprule
& \textbf{Layer Description} & \textbf{K} & \textbf{S} & \textbf{Out. Dim.} \\ 
\toprule
\#0 & Input 2 RGB images & - & - & 6$\times$H$\times$W \\ 
\midrule
\#1  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 16$\times$H/2$\times$W/2 \\
\#2  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 32$\times$H/4$\times$W/4 \\
\#3  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 64$\times$H/8$\times$W/8 \\
\#4  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 128$\times$H/16$\times$W/16 \\
\#5  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 256$\times$H/32$\times$W/32 \\
\#6  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 256$\times$H/64$\times$W/64 \\
\#7  & \hspace{2mm} Conv2d $\shortrightarrow$ GN $\shortrightarrow$ ReLU \hspace{2mm} & 3 & 2 & 256$\times$H/128$\times$W/128 \\
\#8  & Conv2d & 1 & 1 & 6$\times$H/128$\times$W/128 \\
\midrule
\#9  & Global Pooling & - & - & 6 \\
\bottomrule
\end{tabular}
\label{tab:netpose}
}}
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{
\textbf{Neural network architectures used in our proposed FSM framework}. The predicted depth maps are $1 \times H \times W$ tensors, and the predicted poses are $6$-dimensional vectors representing translation ($x,y,z$) and Euler rotation angles (pitch, yaw, roll).  \emph{BN} stands for Batch Normalization \cite{ioffe2015batch}, \emph{GN} for Group Normalization \cite{WuH18}, \emph{Upsample} doubles spatial dimensions using bilinear interpolation, and \emph{ReLU} denote Rectified Linear Units. The symbol $\oplus$ indicates feature concatenation. 
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\label{tab:networks}
%\vspace{-5mm}
\end{table}


==> full_surround_monodepth/tables/table_rot_averaging.tex <==
\captionsetup[table]{skip=6pt}

\begin{table}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.87}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccc}
\toprule
\textbf{Method} & 
Abs Rel$\downarrow$ &
Sq Rel$\downarrow$ &
RMSE$\downarrow$ &
$\delta_{1.25}$ $\uparrow$
\\
\toprule
FSM & 0.133 & 2.817 & \textbf{13.598} & 0.837\\
FSM + PCC (trans only) & 0.132 & 2.826 &  13.805 & 0.836\\
FSM + PCC (rot only) & 0.131 & 2.766 & 13.694 & 0.835 \\
\midrule
\textbf{FSM + PCC} & \textbf{0.130} & \textbf{2.752} & 13.866  & \textbf{0.838} \\
\bottomrule
\end{tabular}
}
\caption{
\textbf{Pose ablation (PCC)} described in Section 3.3. Our method with and without different components of the pose constraint, results on \textbf{F}.}
\label{table:pose-constraint}
\end{table}

==> neural_ray_surfaces/sections/03selfsup.tex <==

In a self-supervised monocular structure-from-motion setting, our goal is to learn: (a) a depth model $f_d: I \to D$, that predicts a depth value $\hat{d} = f_d(I(\mathbf{p}))$ for every pixel $\mathbf{p}=[u, v]^T$ in the target image $I_t$ (up to a scale factor);
and (b) an ego-motion model $f_{\mathbf{x}}: (I_t,I_C) \to \mathbf{X}_{t \to C}$, that predicts the rigid transformations for all $c \in C$ given by $\mathbf{X}_{t \to c} = \begin{psmallmatrix}\mathbf{R} & \mathbf{t}\\ \mathbf{0} & \mathbf{1}\end{psmallmatrix} \in \text{SE(3)}$, between the target image $I_t$ and a set of context images $I_c \in I_C$, i.e. adjacent frames in a video sequence. 

% -------------------------------------------------
\subsection{Objective Function}
\label{sec:preliminaries}
Following the work of Zhou et al.~\cite{zhou2017unsupervised}, we train the depth and pose networks simultaneously in a self-supervised manner. This is achieved by projecting pixels from the context image $I_c$ onto the target image $I_t$, and minimizing the photometric reprojection error between original $I_t$ and synthesized $\hat{I}_t$ images. The image synthesis operation is done using Spatial Transformer Networks (STNs)~\cite{jaderberg2015spatial},  via grid sampling with bilinear interpolation, and is thus fully differentiable. This pixel-wise warping is depicted in Figure~\ref{fig:transforms}a and takes the form of:
\begin{equation}
\hat{\mathbf{p}}_t 
=
\pi_c \big(\mathbf{R}_{t \rightarrow c} \phi_t (\mathbf{p}_t, d_t) + \mathbf{t}_{t \rightarrow c}\big),
\label{eq:recproj}
\end{equation}
%\begin{equation}
%\hat{d}_t \cdot \hat{\mathbf{p}}_t = K_t \big(R_{s \rightarrow t} K_s^{-1} %\mathbf{p}_s \cdot d_t + \mathbf{t}_{s \rightarrow t}\big),
%\end{equation}
where $\phi(\tilde{\mathbf{p}}, d) = \mathbf{P}$ is responsible for the unprojection of an image pixel in homogeneous coordinates $\tilde{\mathbf{p}}=[u, v, 1]^T$ to a 3D point $\mathbf{P}=[x, y, z]^T$ given its depth value $d$. Conversely, $\pi(\mathbf{P}) = \tilde{\mathbf{p}}$ projects a 3D point back onto the image plane as a pixel. For the standard pinhole camera model, used in most of the current learning-based monocular depth estimation algorithms \cite{monodepth2,pillai2018superdepth,yang2017unsupervised,zhan2018unsupervised,zhou2018unsupervised}, these functions have a closed-form solution and can be calculated as:
\begin{equation}
\small
\phi(\tilde{\mathbf{p}}, d) = d \hspace{1mm} \mathbf{K}^{-1} \tilde{\mathbf{p}} =
d 
\left[\begin{array}{ccc}
f_x & 0 & c_x \\
0 & f_y & c_y \\
0 & 0 & 1
\end{array}\right]^{-1} 
\hspace{-3mm}
\left[\begin{array}{ccc}
u & v & 1
\end{array}\right]^T 
\label{eq:pinhole_reconstruction}
\end{equation}
\begin{equation}
\pi(\mathbf{P}) = 
\frac{1}{\mathbf{P}_z}\mathbf{K} \mathbf{P} =
\frac{1}{z} 
\left[\begin{array}{ccc}
f_x & 0 & c_x \\
0 & f_y & c_y \\
0 & 0 & 1
\end{array}\right]
\left[\begin{array}{ccc}
x & y & z
\end{array}\right]^T,
\label{eq:pinhole_projection}
\end{equation}

with intrinsics matrix $\mathbf{K}$, focal length $(f_x, f_y)$ and principal point $(c_x, c_y)$. These parameters are usually assumed to be known, obtained using prior independent calibration techniques, or are learned as additional variables during the training stage \cite{gordon2019depth}. The self-supervised objective loss to be minimized is of the form:
\begin{align}
\small
    \mathcal{L}(I_t,\hat{I_t}) = \mathcal{L}_p(I_t,I_C) +  \lambda_d~\mathcal{L}_d(\hat{D}_t),
    \label{eq:overall-loss}
\end{align}
which is the combination of an appearance-based loss $\mathcal{L}_p$ and a weighted depth smoothness loss $\mathcal{L}_d$, described below in more detail. This loss is then averaged per pixel and batch during training to produce the final value to be minimized.  
For simplicity, unlike many of the recent state-of-the-art methods \cite{gordon2019depth,vijayanarasimhan2017sfm} we do not explicitly model dynamic objects (which break the static scene assumption), although these could be easily incorporated into our framework to further improve experimental results.

% -------------------------------------------------
\textbf{Appearance-Based Loss.}~Similar to Godard et al.~\cite{godard2017unsupervised} and Zhou et al.~\cite{zhou2017unsupervised}, the similarity between target $I_t$ and warped $\hat{I_t}$ images is estimated at the pixel level using Structural Similarity (SSIM)~\cite{wang2004image} combined with an L1 loss term:
\begin{equation}
\small
\mathcal{L}_{p}(I_t,\hat{I_t}) = \alpha~\frac{1 - \text{SSIM}(I_t,\hat{I_t})}{2} + (1-\alpha)~\| I_t - \hat{I_t} \|.
\label{eq:loss-photo}
\end{equation}
To increase robustness against parallax or the presence of dynamic objects, we follow Godard et al.~\cite{monodepth2} and consider only the minimum pixel-wise photometric loss value for each context image in $I_C$.
%The intuition is that the same pixel will not be occluded or out-of-bounds in all context images, and its association with minimal photometric loss should be correct.
Similarly, we mask out static pixels by removing those with warped photometric loss $\mathcal{L}_p(I_t, \hat{I}_t)$ higher than the original photometric loss $\mathcal{L}_p(I_t, I_c)$.


% -------------------------------------------------
\textbf{Depth Smoothness Loss.}~~To regularize the depth in textureless image regions, we incorporate an edge-aware term similar to Godard et al.~\cite{godard2017unsupervised}, that penalizes high depth gradients in areas with low color gradients: %The loss is weighted for each of the pyramid-levels, and is decayed by a factor of 2 on down-sampling, starting with a weight of 1 for the $0^\text{th}$ pyramid level.
\begin{align}
  \mathcal{L}_{s}(\hat{D}_t) = | \delta_x \hat{D}_t | e^{-|\delta_x I_t|} + | \delta_y \hat{D}_t | e^{-|\delta_y I_t|},
  \label{eq:loss-disp-smoothness}
\end{align}


==> neural_ray_surfaces/sections/figure_qualitative.tex <==
%\graphicspath{{figures/}{../figures/}}
\begin{figure*}[h!]
\centering
\subfloat[Pinhole (KITTI)]{
\includegraphics[width=0.2\textwidth,trim={0 16cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/kitti_0000000042.png}
\includegraphics[width=0.2\textwidth,trim={0 16cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/kitti_0000000124.png}
\includegraphics[width=0.2\textwidth,trim={0 16cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/kitti_0000000522.png}
\includegraphics[width=0.2\textwidth,trim={0 16cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/kitti_0000001259.png}
\includegraphics[width=0.2\textwidth,trim={0 16cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/kitti_0000001653.png}}
\begin{comment}
\\
%\vspace{-2mm}
\subfloat[Pinhole (Multi-FOV) \vitor{TODO}]{
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000000005.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000000277.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000000885.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000001536.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000001965.png}}
\end{comment}
\\
%\vspace{-2mm}
\subfloat[Fisheye (Multi-FOV)]{
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000000005.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000000277.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000000885.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000001536.png}
\includegraphics[width=0.16\textwidth,trim={0 0cm 38cm 0}, clip]{neural_ray_surfaces/figures/experiments/fov_fisheye_0000001965.png}}
\\
%\vspace{-2mm}
\subfloat[Catadioptric (OmniCam)]{
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{neural_ray_surfaces/figures/experiments/omnicam_0000011810.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{neural_ray_surfaces/figures/experiments/omnicam_0000010698.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{neural_ray_surfaces/figures/experiments/omnicam_0000001826.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{neural_ray_surfaces/figures/experiments/omnicam_0000000536.png}
\includegraphics[width=0.16\textwidth,height=5.5cm,trim={0 0cm 29cm 0}, clip]{neural_ray_surfaces/figures/experiments/omnicam_0000000086.png}}
\\
% \vspace{-2mm}
\caption{\textbf{Qualitative depth estimation results for different camera geometries} using our proposed NRS framework. Note that all these results were obtained using the same architecture and parameters (Figure \ref{fig:diagram}); the only modification are the video sequences used for training and inference.
}
\label{fig:qualitative}
\end{figure*}


==> neural_ray_surfaces/supp_sections/figure_diagram.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.9\textwidth]{neural_ray_surfaces/figures/theory/diagram3.pdf}
\caption{\textbf{Proposed self-supervised monocular depth, pose and ray surface estimation framework}. Both depth and ray surface decoders share the same encoder backbone, and by combining the predicted depth map $\hat{D}_t$ with the predicted ray surface $\hat{\mathbf{Q}}_t$, we are able to perform the view synthesis necessary for self-supervised learning.}
\label{fig:diagram}
\end{figure}
\vspace{-3mm}
